Synchronous and Asynchronous Parallelism Approaches for Generalized Canonical Polyadic Tensor Decomposition with GenTen

The Canonical Polyadic (CP) tensor decomposition is a well-known method for interpretable analysis of high-dimensional data. Recently, the Generalized CP method (GCP) was introduced by Hong and Kolda to allow for flexible choice of the loss function in the optimization problem defining the CP model, enabling more interpretable decompositions of strongly non-Gaussian data such as count or binary data. Furthermore, Kolda and Hong introduced a version of GCP that leverages randomization and stochastic optimization to address scalability to large, sparse data sets. In this work, we take these ideas a step further and consider synchronous and asynchronous algorithms for parallel GCP tensor decomposition through the GenTen software package, exploiting both shared and distributed memory parallelism. We build on shared memory parallel CP decomposition algorithms utilizing Kokkos for portability across CPU and GPU architectures to support the random sampling and stochastic optimization methods required by GCP. We then couple this approach to the well-known medium-grained distributed memory parallelism scheme developed for traditional CP decompositions through MPI, providing a synchronous, hybrid MPI+Kokkos, parallel GCP decomposition capability. Finally, we propose an asynchronous distributed parallelism approach building on related techniques for federated learning to achieve even better scalability to large data sets. We study the effectiveness of the proposed synchronous and asynchronous approaches vis-a-vis computational cost and accuracy on synthetic and publicly-available real-world datasets of varying sizes, dimensions, and sparsity patterns using several loss functions.

==> gcp.tex <==
% !TEX root = main.tex

%There is growing interest to extend low-rank matrix decompositions to multi-way
%arrays, or \emph{tensors}. One of the most useful low-rank tensor
% decompositions
%is the \emph{canonical polyadic decomposition (CPD)}. The CPD represents a
%tensor as a finite sum of rank-one outer products, a generalization of the
%matrix singular value decomposition (SVD) to tensors.
%
%For example, the rank-$k$ SVD approximation of a matrix $\mat{A} \in \R^{I_1
%\times I_2}$ is
%%written as a 2-dimensional CP tensor decomposition is
%\begin{equation}
%  \mat{A} \approx \mat{U}_1 \mat{\Sigma} \mat{U}_2^T =
%  \sum_{r=1}^k \sigma_r \mat{u}_1(\colon,r) \circ
%  \mat{u}_2(\colon,r),
%\end{equation}
%subject to orthogonality constraints $\mat{U}_1^T\mat{U}_1 =
%\mat{U}_2^T\mat{U}_2 = \mat{I}_k$, where $\mat{I}_k$ is the identity matrix
%with $k$ rows and columns. Note that with $\mat{U}_1 = \mat{U}$ and $\mat{U}_2
%= \mat{V}$ we recover the standard form of the matrix
%SVD~\Cref{eq:svd:full_rank}: $\mat{A} = \mat{U} \mat{\Sigma} \mat{V}^T$. In
%the parlance of CP, $\mat{U}_1$ and $\mat{U}_2$ are \emph{factor matrices}
%corresponding to the first and second \emph{modes} of $\mat{A}$, respectively.
%The column vectors of the factor matrices are referred to as
%\emph{components}; for example, $\mat{U}_1(\colon,1)$ refers to the first
%component of the factor matrix corresponding to the first mode of $\mat{A}$.
%
%One major distinction is that there are no
%orthogonality constraints on the vectors of the CPD model. Thus we treat the
%matrix SVD as a special case of the CPD. Nonetheless, low-rank CP
% decompositions
%are appealing for reasons similar to those of the low-rank SVD, including
%dimensionality reduction, compression, de-noising, and more.
% Interpretability of
%CP decompositions on real problems is well-documented, with applications
%including exploratory temporal data analysis and link
%prediction~\cite{Dunlavy11TemporalLinkPrediction},
%chemometrics~\cite{Mocks88TopographicComponentsModel}, neuroscience
%\cite{Andersen03PracticalAspectsPARAFAC}, and social network and web link
%analysis~\cite{Kolda05HigherorderWebLink,
%Kolda09TensorDecompositionsApplications}.
%
%One particular application of interest is when the tensor data are counts. In
%this case, a common modeling choice is to assume that the data follow a Poisson
%distribution so that statistical methods, like maximum likelihood estimation,
%can be applied to the analysis. One key challenge for computing the Poisson CPD
%is that a low-rank CP tensor model of Poisson parameters must satisfy certain
%nonnegativity and stochasticity constraints. In the next few sections we cover
%the details of the low-rank CP tensor models of Poisson parameters and
%decompositions which are the focus of this work.

\subsection{Low-rank CP tensor model}
Assume $\tns{X}$ is a $d$-way tensor of size $I_1 \times \dots \times I_d$. The
tensor $\tns{X}$ is rank-one if it can be expressed as the outer product of $d$
vectors, each corresponding to a mode in $\tns{X}$, i.e.,
\begin{equation}
  \label{eq:cp:rank_one}
  \tns{X} = \mat{a}_1 \circ \mat{a}_2 \circ \dots \circ \mat{a}_d.
\end{equation}
More broadly, the \emph{rank} of a tensor $\tns{X}$ is the smallest number of
rank-one tensors that generate $\tns{X}$ as their
sum~\cite{Kolda09TensorDecompositionsApplications}. We concentrate on the
problem of approximating a tensor of data with a low-rank CP tensor model, i.e.,
the sum of relatively few rank-one tensors.

Let $\bm{\lambda} = [\lambda_1, \lambda_2, \ldots, \lambda_d]\in\R^d$ be a
vector of scalars and let $\mat{A}_1 \in\R^{I_1 \times R}$, $\mat{A}_2 \in
\R^{I_2\times R}$, $\ldots,$ $\mat{A}_d \in \R^{I_d \times R}$ be matrices. The
\emph{rank-$R$ canonical polyadic (CP) tensor model of
$\tns{X}$}~\cite{Harshman70FoundationsPARAFACProcedure,
Carroll70AnalysisIndividualDifferences} is:
\begin{equation}
  \label{eq:cp}
  \tns{X} \approx \tns{M}
  = \llbracket \bm{\lambda}; \mat{A}_1, \ldots, \mat{A}_d \rrbracket
  \coloneqq \sum_{r=1}^R \lambda_r \mat{A}_1(\colon,r) \circ \dots
  \circ \mat{A}_d(\colon,r).
\end{equation}
Each $\mat{A}_k \in \R^{I_k \times R}$ is a \emph{factor matrix} with $I_k$ rows
and $R$ columns. The $j$-th \emph{component} of the mode-$k$ factor matrix is
the column vector $\mat{A}_k(\colon,j)$. We refer to the form $\tns{M} =
\llbracket \bm{\lambda}; \, \mat{A}_1, \ldots, \mat{A}_d \rrbracket$ as a
\emph{Kruskal tensor}.

%\subsection{Computing the Poisson CPD for count data}
%\label{sec:background:cp:nntf}
%We focus on an application where all of the entries in a data tensor
% are counts.
%For the remainder of this work, let $\tns{X} \in \Z_+^{I_1 \times \dots \times
%I_d}$ be a $d$-way tensor of nonnegative integers, let $\tns{M}$ be a CP tensor
%model of the form~\Cref{eq:cp}, and assume the following about $\tns{X}$:
%\begin{itemize}
%\item each $x_{\mind} \in \tns{X}$ is sampled from a Poisson distribution
%  with parameter $m_{\mind}\in \tns{M}$, and
%\item the tensor $\tns{X}$ has low-rank structure (i.e., $R <
%  \sqrt[d]{\prod_{k=1}^d I_k}$~\cite{Kolda20StochasticGradientsLargeScale}).
%\end{itemize}%
%Chi and Kolda showed in~\cite{Chi12TensorsSparsityNonnegative} that
%under
%the assumptions above%
%a \emph{Poisson CP tensor model} is an effective low-rank
%approximation of
%a tensor of counts, $\tns{X}$, and presented an algorithm for computing
%$\tns{M}$.%
%The Poisson CP tensor model has shown to be
%valuable in analyzing latent patterns and relationships in count data across
%many application areas, including food
%production~\cite{Bro98MultiwayAnalysisFood}, network
%analysis~\cite{Dunlavy11MultilinearAlgebraAnalyzing,
%Baskaran19EnhancingNetworkVisibility}, term-document
%analysis~\cite{Chew07CrosslanguageInformationRetrieval,
%Henretty18TopicModelingAnalysis}, email
% analysis~\cite{Bader08SurveyTextMining},
%link prediction~\cite{Dunlavy11TemporalLinkPrediction}, geospatial
%analysis~\cite{Ezick19CombiningTensorDecompositions,
%Henretty17QuantitativeQualitativeAnalysis}, and web page
%analysis~\cite{Kolda06TOPHITSModelHigherorder}.
%
%One numerical approach to fit a low-rank Poisson CP tensor model to data is
%\emph{tensor maximum likelihood estimation}, which has proven to be successful.
%Computing the Poisson CPD via tensor maximum likelihood estimation involves
%minimizing the following nonlinear, nonconvex optimization problem:
%\begin{equation}
%  \label{eq:hybrid-gc:background:nll}
%  \min_{\tns{M}} f\left( \tns{X}, \tns{M} \right) =
%  \min \sum_{\mind} m_{\mind} - x_{\mind} \log
%  m_{\mind},
%\end{equation}
%where $\mind$ is the multi-index~\Cref{eq:cp:multi-index},
% $x_{\mind} \geq 0$ is
%an entry in $\tns{X}$, and $m_{\mind} > 0$ is a parameter in the Poisson CP
%tensor model $\tns{M}$. The function $f(\tns{X},\tns{M})$
%in~\Cref{eq:hybrid-gc:background:nll} is the negative of the log-likelihood of
%the Poisson distribution (omitting the constant
%$\sum_{\mind}\log\left(x_{\mind}!\right)$
%term)~\cite{Rodriguez07PoissonModelsCount}. We will refer to it simply as
%\emph{Poisson loss}.
%
%In contrast to linear maximum likelihood
%estimation~\cite{Myung03TutorialMaximumLikelihood}, where a single parameter is
%estimated using multiple data instances, tensor maximum likelihood estimation
%fits a single parameter in an approximate low-rank model to a single data
%instance. Within the tensor context, low-rank structure means that multiple
%instances in the data are linked to a single model parameter, a type of
%multilinear maximum likelihood estimation. This distinction is not
% made anywhere
%else in the literature, to the best of our knowledge.
%
%Much of the research associated with computing the low-rank Poisson CPD via
%tensor maximum likelihood estimation has focused on local
%methods~\cite{Chi12TensorsSparsityNonnegative,
%Hansen15NewtonbasedOptimizationKullback, Hong20GeneralizedCanonicalPolyadic,
%Kolda20StochasticGradientsLargeScale}, particularly with respect to
%computational performance~\cite{Teranishi20SparTenLeveragingKokkos,
%Myers20ParameterSensitivityAnalysis,
%Phipps19SoftwareSparseTensor,Baskaran19FastScalableDistributed,
%Letourneau18ComputationallyEfficientCP,
% Baskaran17MemoryefficientParallelTensor,
%Baskaran14LowoverheadLoadbalancedScheduling}. Many of the current local methods
%for Poisson CPD can be classified as either an
%\emph{alternating}~\cite{Carroll70AnalysisIndividualDifferences,
%Harshman70FoundationsPARAFACProcedure} or an
%\emph{all-at-once}~\cite{Acar11ScalableOptimizationApproach,
%Acar11AllatonceOptimizationCoupled,Phan13LowComplexityDamped} optimization
%method.
%
%Alternating local methods iteratively solve a series of subproblems by fitting
%each factor matrix sequentially while the remaining factor matrices are held
%fixed. These methods are a form of coordinate descent
%(CD)~\cite{Wright15CoordinateDescentAlgorithms}, where each factor matrix is a
%block of components that is fit while the remaining component blocks (i.e.,
%factor matrices) are left unchanged. Since each block corresponds to a
%lower-dimensional problem, alternating tensor methods employ block CD
%iteratively to solve a series of easier problems.  CP Alternating Poisson
%Regression (CPAPR) was introduced by Chi and Kolda
%in~\cite{Chi12TensorsSparsityNonnegative} as a nonlinear Gauss-Seidel approach
%to block CD that uses a fixed-point majorization-minimization algorithm called
%\emph{Multiplicative Updates (CPAPR-MU)}. At the highest level, the CPAPR
%algorithm performs an \textit{outer iteration} where optimizations are applied
%on each mode in an alternating fashion. An \emph{inner iteration} is an
%optimization using multiplicative updates applied to a subset of variables
%corresponding to an individual mode. Inner iterations are performed until the
%convergence criterion is satisfied for a mode or up to the maximum allowable
%number, $l_{max}$. Outer iterations are performed until the convergence
%criterion is satisfied for the whole model or up to the maximum allowable
%number, $k_{max}$. The convergence criterion is based on the
%\emph{Karush-Kuhn-Tucker (KKT)} conditions, necessary conditions for
% convergence
%to a local minimum in nonlinear optimization. A local minimizer that satisfies
%the KKT conditions is called a \emph{KKT point}.
%
%Hansen et al. in~\cite{Hansen15NewtonbasedOptimizationKullback} presented two
%Newton-based, active set gradient projection methods using up to second-order
%information, \emph{Projected Damped Newton (CPAPR-PDN)} and \emph{Projected
%Quasi-Newton (CPAPR-PQN)}. Moreover, they provided extensions to these methods
%where each component block of the CPAPR minimization can be further separated
%into independent, highly-parallelizable row-wise subproblems; these methods are
%\emph{Projected Damped Newton for the Row subproblem (CPAPR-PDNR)}
%and \emph{Projected Quasi-Newton for the Row subproblem (CPAPR-PQNR)}.
%
%One outer iteration of all-at-once optimization methods updates all
% optimization
%variables simultaneously. The Generalized Canonical Polyadic decomposition
%algorithm (GCP)~\cite{Hong20GeneralizedCanonicalPolyadic} is a gradient descent
%method based on a generic formulation of first derivative information for
%arbitrary loss functions to compute the CPD via tensor maximum likelihood
%estimation. The original GCP method has two variants: 1) deterministic, which
%uses limited-memory quasi-Newton optimization (L-BFGS) and 2) stochastic, which
%supports gradient descent (SGD),
%AdaGrad~\cite{Duchi11AdaptiveSubgradientMethods}, and
%Adam~\cite{Kingma15AdamMethodStochastic} optimizations. The stochastic variants
%perform loss function and gradient computations on samples of the input data
%tensor so that the search path is computed from estimates of these values. We
%focus here on GCP-Adam~\cite{Kolda20StochasticGradientsLargeScale}, which
%applies Adam for scalability.
%
%More generally, we focus on the GCP and CPAPR families of tensor maximum
%likelihood-based local methods for Poisson CPD for the following reasons:
%\begin{enumerate}
%
%  \item \emph{Existing Theory}: Method convergence, computational costs, and
%        memory demands are well-understood.
%
%  \item \emph{Available Software}: High-level MATLAB implementing both
%        families is available in MATLAB Tensor Toolbox
%        (TTB)\footnote{\url{https://gitlab.com/tensors/tensor_toolbox}.}~\cite{Bader17MATLABTensorToolbox,Bader08EfficientMATLABComputations}.
%        A Python version is available in
%        pyttb.\footnote{\url{https://github.com/sandialabs/pyttb}.} High
%        performance C++ code that leverages the Kokkos hardware abstraction
%        library~\cite{Kokkos} to provide parallel computation on diverse
%        computer architectures (e.g., x86-multicore, GPU, etc.) is available
%        with SparTen\footnote{\url{https://github.com/sandialabs/sparten}.}
%        for CPAPR~\cite{Teranishi20SparTenLeveragingKokkos} and
%        Genten\footnote{\url{https://gitlab.com/tensors/genten}.} for
%        GCP~\cite{Phipps19SoftwareSparseTensor}. Additional open-source
%        software for MATLAB includes N-Way
%        Toolbox~\cite{Andersson00NwayToolboxMatlab} and
%        Tensorlab~\cite{Vervliet16TensorlabNumericalOptimization}. Commercial
%        software includes ENSIGN Tensor Toolbox~\cite{Baskaran22ENSIGN}.
%\end{enumerate}

%\subsection{Related work}
%There are other approaches in the literature that seek to fit models with other
%distributions in the exponential family or that use other algorithms
% to estimate
%parameters. Alternating least squares methods are relatively easy to implement
%and effective when used with LASSO-type
%regularization~\cite{Friedlander08ComputingNonnegativeTensor,
%Bazerque13InferencePoissonCount}. The method of Ranadive et
%al.~\cite{Ranadive21AllOnceCP}, CP-POPT-DGN, is an all-at-once active set
%trust-region gradient-projection method. CP-POPT-DGN is functionally very
%similar to CPAPR-PDN. Whereas CP-POPT-DGN computes the search direction via
%preconditioned conjugate gradient (PCG), CPAPR-PDNR computes the search
%direction via Cholesky factorization. The most significant differences are: 1)
%CP-POPT-DGN is all-at-once whereas all CPAPR methods are alternating and 2)
%CPAPR can take advantage of the separable row subproblem formulation to achieve
%more fine-grained parallelism. The Generalized Gauss-Newton method of
%Vandecapelle et al.~\cite{Vandecappelle20SecondorderMethodFitting} follows the
%GCP framework to fit arbitrary non-least squares loss via an all-at-once
%optimization and trust-region-based Gauss-Newton approach.  Hu et
%al.~\cite{Hu15ScalableBayesianNonnegative, Hu15ZeroTruncatedPoissonTensor}
%re-parameterized the Poisson regression problem to leverage Gibbs sampling and
%variational Bayesian inference to account for the inability of CPAPR to handle
%missing data. Other problem transformations include probabilistic likelihood
%extensions via Expectation Maximization~\cite{Rai15ScalableProbabilisticTensor,
%Huang17KullbackLeiblerPrincipalComponent} and a Legendre
%decomposition~\cite{Sugiyama18LegendreDecompositionTensors} instead of a CP
%decomposition.

%\subsection{Factor match score}
%\label{ch:background:cp:fms}
%\input{chapters/etc/fms}


==> images/tensor3d.tex <==

% Define Royal Blue using CMYK values
\definecolor{myblue}{cmyk}{0.71, 0.53, 0.00, 0.12}
\definecolor{myorange}{cmyk}{0.00, 0.35, 1.00, 0.00}
\definecolor{myred}{cmyk}{0.00, 0.93, 0.93, 0.19}

\draw[white, thick] (origin) -- (lowerfrontleft) -- (lowerfrontright) -- (lowerbackright) -- cycle;% Bottom Face
\draw[white, thick] (origin) -- (upperbackleft) -- (upperbackright) -- (lowerbackright) -- cycle;% Back Face
\draw[white, thick] (origin) -- (upperbackleft) -- (upperfrontleft) -- (lowerfrontleft) -- cycle;% Left Face
\draw[white, thick, fill=gray] (lowerbackright) -- (upperbackright) -- (upperfrontright) -- (lowerfrontright) -- cycle;% Right Face
\draw[white, thick, fill=gray!75] (lowerfrontleft) -- (upperfrontleft) -- (upperfrontright) -- (lowerfrontright) -- cycle;% Front Face
\draw[white, thick, fill=gray!62.5] (upperbackleft) -- (upperfrontleft) -- (upperfrontright) -- (upperbackright) -- cycle;% Top Face

% Front face grid lines
\draw[white, thick] ($ (lowerfrontleft)!.33!(lowerfrontright)$) -- ($ (upperfrontleft)!.33!(upperfrontright)$);
\draw[white, thick] ($ (lowerfrontleft)!.67!(lowerfrontright)$) -- ($ (upperfrontleft)!.67!(upperfrontright)$);
\draw[white, thick] ($ (upperfrontleft)!.5!(lowerfrontleft)$) -- ($ (upperfrontright)!.5!(lowerfrontright)$);

% Top face grid lines
\draw[white, thick] ($ (upperfrontleft)!.33!(upperfrontright)$) -- ($ (upperbackleft)!.33!(upperbackright)$);
\draw[white, thick] ($ (upperfrontleft)!.67!(upperfrontright)$) -- ($ (upperbackleft)!.67!(upperbackright)$);
\draw[white, thick] ($ (upperfrontleft)!.5!(upperbackleft)$) -- ($ (upperfrontright)!.5!(upperbackright)$);

% Right face grid lines
\draw[white, thick] ($ (upperfrontright)!.5!(lowerfrontright)$) -- ($ (upperbackright)!.5!(lowerbackright)$);
\draw[white, thick] ($ (upperfrontright)!.5!(upperbackright)$) -- ($ (lowerfrontright)!.5!(lowerbackright)$);

% Accent front/bottom/right element
\draw[white, thick, fill=myred!85] ($ (lowerfrontleft)!.67!(lowerfrontright)$) -- (lowerfrontright) -- ($ (lowerfrontright) +
(0,0.5*\Height,0) $) -- ($(lowerfrontleft)!.67!(lowerfrontright) + (0, 0.5*\Height,0) $) -- cycle;
\draw[white, thick, fill=myred] (lowerfrontright) -- ($ (lowerfrontright)!.5!(lowerbackright) $) -- ($(lowerfrontright)!.5!(lowerbackright) +
(0,0.5*\Height,0)$) -- ($ (lowerfrontright) + (0,0.5*\Height,0) $) -- cycle;

==> notation.tex <==
% !TEX root = main.tex

A tensor $\tns{X}$ is a $d$-way array with dimensions $I_1 \times I_2
\times \dots \times I_d$. The
\emph{rank-$R$ canonical polyadic (CP) tensor model of
$\tns{X}$}~\cite{Harshman70FoundationsPARAFACProcedure,
Carroll70AnalysisIndividualDifferences} is:
\begin{equation}
  \label{eq:cp}
  \tns{X} \approx \tns{M}
  = \llbracket \mat{A}_1, \ldots, \mat{A}_d \rrbracket
  \coloneqq \sum_{r=1}^R \mat{A}_1(\colon,r) \circ \dots
  \circ \mat{A}_d(\colon,r).
\end{equation}
Each $\mat{A}_k \in \R^{I_k \times R}$ is a \emph{factor matrix} with $I_k$ rows
and $R$ columns. The $j$-th \emph{component} of the mode-$k$ factor matrix is
the column vector $\mat{A}_k(\colon,j)$.
% We refer to the form $\tns{M} = \llbracket \bm{\lambda}; \,
% \mat{A}_1, \ldots, \mat{A}_d \rrbracket$ as a \emph{Kruskal tensor}.

% The set of real numbers and integers are denoted as $\R$ and $\Z$,
% respectively.
% The real numbers and integers restricted to nonnegative values are denoted as
% $\R_+$ and $\Z_+$, respectively.
% The \emph{order} of a tensor is the number of
% \textit{dimensions} or \textit{ways}. Each tensor dimension is called a
% \textit{mode}. A scalar is represented by a lowercase
% letter, e.g., $x$. A bold lowercase letter denotes a vector, e.g.,
% $\mat{v}$. A matrix is denoted by a bold
% capital letter, e.g., $\mat{A} \in \R^{m \times n}$. Tensors of
% order three and
% higher are expressed with a bold capital script letter, e.g.,
% $\tns{X} \in \R^{m
% \times n \times p}$.  Estimated or approximated values are
% typically written with a tilde.

% The $i$-th entry of a vector $\vec{v}$ is denoted $v_i$, the
% $(i,j)$ entry of a
% matrix $\mat{M}$ is denoted $m_{ij}$, and the $(i,j,k)$ entry of a three-way
% tensor $\tns{X}$ is denoted $x_{ijk}$. \emph{Fibers} are the higher-order
% analogue of matrix rows and columns. Indices are integer values
% that range from
% 1 to a value denoted by the capitalized version of the index
% variable, e.g., $i
% = 1,\ldots,I$.  We use MATLAB-style notation for subarrays formed
% from a subset
% of indices of a vector, matrix, or tensor mode.  We use the shorthand $i_j
% \colon i_k$ when the subset of indices forming a subarray is the range
% $i_j,\ldots,i_k$. The special case of a colon $\colon$ by itself indicates all
% elements of a mode, e.g., the $j$-th column or mode-1 fiber of the matrix
% $\mat{A}$ is $\mat{A}(\colon,j) = \mat{A}(i_1 \colon i_{I}, j)$. We use the
% \textit{multi-index}
% % \begin{equation}
% %   \label{eq:cp:multi-index} \mind \coloneqq (i_1, i_2, \ldots, i_d)
% %   \eqwith i_j \in \{1, 2,\ldots,I_j\} \eqfor j = 1,\ldots,d,
% % \end{equation}
% as a convenient shorthand for the $(i_1, i_2, \ldots, i_d)$ entry of a $d$-way
% tensor.

% Superscript $T$ denotes non-conjugate matrix transpose. We assume vectors
% $\vec{u}$ and $\vec{v}$ are column vectors so that $\vec{u}^T\vec{v}$ is an
% inner product of vectors and $\vec{u}\vec{v}^T$ is an outer product
% of vectors.
% We also denote outer products of vectors as $\vec{u} \circ \vec{v} = \vec{u}
% \vec{v}^T$, which is especially useful when describing the outer
% products of more than two vectors. The number of matrix or tensor non-zero
% elements is denoted $\nnz(\cdot)$; conversely, the number of zeros in a matrix
% or tensor is denoted $\nz(\cdot)$.

% \subsection{Matricization: transforming a tensor into a matrix}
% \textit{Matricization}, as defined
% in~\cite{Kolda09TensorDecompositionsApplications}, also known as
% \textit{unfolding} or \textit{flattening}, is the process of reordering the
% elements of a $d$-way array into a matrix. The mode-$n$ matricization of a
% tensor $\tns{X} \in \R^{I_1 \times I_2 \times \dots \times I_d}$, denoted
% $\mat{X}_{(n)}$, arranges the mode-$n$ fibers to be the columns of
% the resulting
% matrix.

